First Measurement of the Decay Asymmetry in the pure W-boson-exchange Decay $\Lambda_{c}^{+}\to\Xi^{0}K^{+}$

Based on $4.4~\text{fb}^{-1}$ of $e^{+}e^{-}$ annihilation data collected at the center-of-mass energies between $4.60$ and $4.70~\text{GeV}$ with the BESIII detector at the BEPCII collider, the pure \textit{W}-boson-exchange decay $\Lambda_{c}^{+}\to\Xi^{0}K^{+}$ is studied with a full angular analysis. The corresponding decay asymmetry is measured for the first time to be $\alpha_{\Xi^{0}K^{+}}=0.01\pm0.16({\rm stat.})\pm0.03({\rm syst.})$. This result reflects the non-interference effect between the $S$- and $P$-wave amplitudes. The phase shift between $S$- and $P$-wave amplitudes has two solutions, which are $\delta_{p}-\delta_{s}=-1.55\pm0.25({\rm stat.})\pm0.05({\rm syst.})~\text{rad}$ or $1.59\pm0.25({\rm stat.})\pm0.05({\rm syst.})~\text{rad}$.

==> author_bk.tex <==
\author{
\begin{small}
\begin{center}
M.~Ablikim$^{1}$, M.~N.~Achasov$^{5,b}$, P.~Adlarson$^{74}$, X.~C.~Ai$^{80}$, R.~Aliberti$^{35}$, A.~Amoroso$^{73a,73c}$, M.~R.~An$^{39}$, Q.~An$^{70,57}$, Y.~Bai$^{56}$, O.~Bakina$^{36}$, I.~Balossino$^{29a}$, Y.~Ban$^{46,g}$, V.~Batozskaya$^{1,44}$, K.~Begzsuren$^{32}$, N.~Berger$^{35}$, M.~Berlowski$^{44}$, M.~Bertani$^{28a}$, D.~Bettoni$^{29a}$, F.~Bianchi$^{73a,73c}$, E.~Bianco$^{73a,73c}$, A.~Bortone$^{73a,73c}$, I.~Boyko$^{36}$, R.~A.~Briere$^{6}$, A.~Brueggemann$^{67}$, H.~Cai$^{75}$, X.~Cai$^{1,57}$, A.~Calcaterra$^{28a}$, G.~F.~Cao$^{1,62}$, N.~Cao$^{1,62}$, S.~A.~Cetin$^{61a}$, J.~F.~Chang$^{1,57}$, T.~T.~Chang$^{76}$, W.~L.~Chang$^{1,62}$, G.~R.~Che$^{43}$, G.~Chelkov$^{36,a}$, C.~Chen$^{43}$, Chao~Chen$^{54}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,62}$, M.~L.~Chen$^{1,57,62}$, S.~J.~Chen$^{42}$, S.~M.~Chen$^{60}$, T.~Chen$^{1,62}$, X.~R.~Chen$^{31,62}$, X.~T.~Chen$^{1,62}$, Y.~B.~Chen$^{1,57}$, Y.~Q.~Chen$^{34}$, Z.~J.~Chen$^{25,h}$, W.~S.~Cheng$^{73c}$, S.~K.~Choi$^{11}$, X.~Chu$^{43}$, G.~Cibinetto$^{29a}$, S.~C.~Coen$^{4}$, F.~Cossio$^{73c}$, J.~J.~Cui$^{49}$, H.~L.~Dai$^{1,57}$, J.~P.~Dai$^{78}$, A.~Dbeyssi$^{18}$, R.~ E.~de Boer$^{4}$, D.~Dedovich$^{36}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{35}$, I.~Denysenko$^{36}$, M.~Destefanis$^{73a,73c}$, F.~De~Mori$^{73a,73c}$, B.~Ding$^{65,1}$, X.~X.~Ding$^{46,g}$, Y.~Ding$^{40}$, Y.~Ding$^{34}$, J.~Dong$^{1,57}$, L.~Y.~Dong$^{1,62}$, M.~Y.~Dong$^{1,57,62}$, X.~Dong$^{75}$, M.~C.~Du$^{1}$, S.~X.~Du$^{80}$, Z.~H.~Duan$^{42}$, P.~Egorov$^{36,a}$, Y.H.~Y.~Fan$^{45}$, Y.~L.~Fan$^{75}$, J.~Fang$^{1,57}$, S.~S.~Fang$^{1,62}$, W.~X.~Fang$^{1}$, Y.~Fang$^{1}$, R.~Farinelli$^{29a}$, L.~Fava$^{73b,73c}$, F.~Feldbauer$^{4}$, G.~Felici$^{28a}$, C.~Q.~Feng$^{70,57}$, J.~H.~Feng$^{58}$, K~Fischer$^{68}$, M.~Fritsch$^{4}$, C.~Fritzsch$^{67}$, C.~D.~Fu$^{1}$, J.~L.~Fu$^{62}$, Y.~W.~Fu$^{1}$, H.~Gao$^{62}$, Y.~N.~Gao$^{46,g}$, Yang~Gao$^{70,57}$, S.~Garbolino$^{73c}$, I.~Garzia$^{29a,29b}$, P.~T.~Ge$^{75}$, Z.~W.~Ge$^{42}$, C.~Geng$^{58}$, E.~M.~Gersabeck$^{66}$, A~Gilman$^{68}$, K.~Goetzen$^{14}$, L.~Gong$^{40}$, W.~X.~Gong$^{1,57}$, W.~Gradl$^{35}$, S.~Gramigna$^{29a,29b}$, M.~Greco$^{73a,73c}$, M.~H.~Gu$^{1,57}$, C.~Y~Guan$^{1,62}$, Z.~L.~Guan$^{22}$, A.~Q.~Guo$^{31,62}$, L.~B.~Guo$^{41}$, M.~J.~Guo$^{49}$, R.~P.~Guo$^{48}$, Y.~P.~Guo$^{13,f}$, A.~Guskov$^{36,a}$, T.~T.~Han$^{49}$, W.~Y.~Han$^{39}$, X.~Q.~Hao$^{19}$, F.~A.~Harris$^{64}$, K.~K.~He$^{54}$, K.~L.~He$^{1,62}$, F.~H~H..~Heinsius$^{4}$, C.~H.~Heinz$^{35}$, Y.~K.~Heng$^{1,57,62}$, C.~Herold$^{59}$, T.~Holtmann$^{4}$, P.~C.~Hong$^{13,f}$, G.~Y.~Hou$^{1,62}$, X.~T.~Hou$^{1,62}$, Y.~R.~Hou$^{62}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,62}$, J.~F.~Hu$^{55,i}$, T.~Hu$^{1,57,62}$, Y.~Hu$^{1}$, G.~S.~Huang$^{70,57}$, K.~X.~Huang$^{58}$, L.~Q.~Huang$^{31,62}$, X.~T.~Huang$^{49}$, Y.~P.~Huang$^{1}$, T.~Hussain$^{72}$, N~H\"usken$^{27,35}$, W.~Imoehl$^{27}$, J.~Jackson$^{27}$, S.~Jaeger$^{4}$, S.~Janchiv$^{32}$, J.~H.~Jeong$^{11}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{19}$, X.~B.~Ji$^{1,62}$, X.~L.~Ji$^{1,57}$, Y.~Y.~Ji$^{49}$, X.~Q.~Jia$^{49}$, Z.~K.~Jia$^{70,57}$, H.~J.~Jiang$^{75}$, P.~C.~Jiang$^{46,g}$, S.~S.~Jiang$^{39}$, T.~J.~Jiang$^{16}$, X.~S.~Jiang$^{1,57,62}$, Y.~Jiang$^{62}$, J.~B.~Jiao$^{49}$, Z.~Jiao$^{23}$, S.~Jin$^{42}$, Y.~Jin$^{65}$, M.~Q.~Jing$^{1,62}$, T.~Johansson$^{74}$, X.~K.$^{1}$, S.~Kabana$^{33}$, N.~Kalantar-Nayestanaki$^{63}$, X.~L.~Kang$^{10}$, X.~S.~Kang$^{40}$, R.~Kappert$^{63}$, M.~Kavatsyuk$^{63}$, B.~C.~Ke$^{80}$, A.~Khoukaz$^{67}$, R.~Kiuchi$^{1}$, R.~Kliemt$^{14}$, O.~B.~Kolcu$^{61a}$, B.~Kopf$^{4}$, M.~Kuessner$^{4}$, A.~Kupsc$^{44,74}$, W.~K\"uhn$^{37}$, J.~J.~Lane$^{66}$, P. ~Larin$^{18}$, A.~Lavania$^{26}$, L.~Lavezzi$^{73a,73c}$, T.~T.~Lei$^{70,k}$, Z.~H.~Lei$^{70,57}$, H.~Leithoff$^{35}$, M.~Lellmann$^{35}$, T.~Lenz$^{35}$, C.~Li$^{47}$, C.~Li$^{43}$, C.~H.~Li$^{39}$, Cheng~Li$^{70,57}$, D.~M.~Li$^{80}$, F.~Li$^{1,57}$, G.~Li$^{1}$, H.~Li$^{70,57}$, H.~B.~Li$^{1,62}$, H.~J.~Li$^{19}$, H.~N.~Li$^{55,i}$, Hui~Li$^{43}$, J.~R.~Li$^{60}$, J.~S.~Li$^{58}$, J.~W.~Li$^{49}$, K.~L.~Li$^{19}$, Ke~Li$^{1}$, L.~J~Li$^{1,62}$, L.~K.~Li$^{1}$, Lei~Li$^{3}$, M.~H.~Li$^{43}$, P.~R.~Li$^{38,j,k}$, Q.~X.~Li$^{49}$, S.~X.~Li$^{13}$, T. ~Li$^{49}$, W.~D.~Li$^{1,62}$, W.~G.~Li$^{1}$, X.~H.~Li$^{70,57}$, X.~L.~Li$^{49}$, Xiaoyu~Li$^{1,62}$, Y.~G.~Li$^{46,g}$, Z.~J.~Li$^{58}$, C.~Liang$^{42}$, H.~Liang$^{1,62}$, H.~Liang$^{70,57}$, H.~Liang$^{34}$, Y.~F.~Liang$^{53}$, Y.~T.~Liang$^{31,62}$, G.~R.~Liao$^{15}$, L.~Z.~Liao$^{49}$, Y.~P.~Liao$^{1,62}$, J.~Libby$^{26}$, A. ~Limphirat$^{59}$, D.~X.~Lin$^{31,62}$, T.~Lin$^{1}$, B.~J.~Liu$^{1}$, B.~X.~Liu$^{75}$, C.~Liu$^{34}$, C.~X.~Liu$^{1}$, F.~H.~Liu$^{52}$, Fang~Liu$^{1}$, Feng~Liu$^{7}$, G.~M.~Liu$^{55,i}$, H.~Liu$^{38,j,k}$, H.~M.~Liu$^{1,62}$, Huanhuan~Liu$^{1}$, Huihui~Liu$^{21}$, J.~B.~Liu$^{70,57}$, J.~L.~Liu$^{71}$, J.~Y.~Liu$^{1,62}$, K.~Liu$^{1}$, K.~Y.~Liu$^{40}$, Ke~Liu$^{22}$, L.~Liu$^{70,57}$, L.~C.~Liu$^{43}$, Lu~Liu$^{43}$, M.~H.~Liu$^{13,f}$, P.~L.~Liu$^{1}$, Q.~Liu$^{62}$, S.~B.~Liu$^{70,57}$, T.~Liu$^{13,f}$, W.~K.~Liu$^{43}$, W.~M.~Liu$^{70,57}$, X.~Liu$^{38,j,k}$, Y.~Liu$^{38,j,k}$, Y.~Liu$^{80}$, Y.~B.~Liu$^{43}$, Z.~A.~Liu$^{1,57,62}$, Z.~Q.~Liu$^{49}$, X.~C.~Lou$^{1,57,62}$, F.~X.~Lu$^{58}$, H.~J.~Lu$^{23}$, J.~G.~Lu$^{1,57}$, X.~L.~Lu$^{1}$, Y.~Lu$^{8}$, Y.~P.~Lu$^{1,57}$, Z.~H.~Lu$^{1,62}$, C.~L.~Luo$^{41}$, M.~X.~Luo$^{79}$, T.~Luo$^{13,f}$, X.~L.~Luo$^{1,57}$, X.~R.~Lyu$^{62}$, Y.~F.~Lyu$^{43}$, F.~C.~Ma$^{40}$, H.~L.~Ma$^{1}$, J.~L.~Ma$^{1,62}$, L.~L.~Ma$^{49}$, M.~M.~Ma$^{1,62}$, Q.~M.~Ma$^{1}$, R.~Q.~Ma$^{1,62}$, R.~T.~Ma$^{62}$, X.~Y.~Ma$^{1,57}$, Y.~Ma$^{46,g}$, Y.~M.~Ma$^{31}$, F.~E.~Maas$^{18}$, M.~Maggiora$^{73a,73c}$, S.~Malde$^{68}$, Q.~A.~Malik$^{72}$, A.~Mangoni$^{28b}$, Y.~J.~Mao$^{46,g}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{73a,73c}$, Z.~X.~Meng$^{65}$, J.~G.~Messchendorp$^{14,63}$, G.~Mezzadri$^{29a}$, H.~Miao$^{1,62}$, T.~J.~Min$^{42}$, R.~E.~Mitchell$^{27}$, X.~H.~Mo$^{1,57,62}$, N.~Yu.~Muchnoi$^{5,b}$, J.~Muskalla$^{35}$, Y.~Nefedov$^{36}$, F.~Nerling$^{18,d}$, I.~B.~Nikolaev$^{5,b}$, Z.~Ning$^{1,57}$, S.~Nisar$^{12,l}$, Y.~Niu $^{49}$, S.~L.~Olsen$^{62}$, Q.~Ouyang$^{1,57,62}$, S.~Pacetti$^{28b,28c}$, X.~Pan$^{54}$, Y.~Pan$^{56}$, A.~~Pathak$^{34}$, P.~Patteri$^{28a}$, Y.~P.~Pei$^{70,57}$, M.~Pelizaeus$^{4}$, H.~P.~Peng$^{70,57}$, K.~Peters$^{14,d}$, J.~L.~Ping$^{41}$, R.~G.~Ping$^{1,62}$, S.~Plura$^{35}$, S.~Pogodin$^{36}$, V.~Prasad$^{33}$, F.~Z.~Qi$^{1}$, H.~Qi$^{70,57}$, H.~R.~Qi$^{60}$, M.~Qi$^{42}$, T.~Y.~Qi$^{13,f}$, S.~Qian$^{1,57}$, W.~B.~Qian$^{62}$, C.~F.~Qiao$^{62}$, J.~J.~Qin$^{71}$, L.~Q.~Qin$^{15}$, X.~P.~Qin$^{13,f}$, X.~S.~Qin$^{49}$, Z.~H.~Qin$^{1,57}$, J.~F.~Qiu$^{1}$, S.~Q.~Qu$^{60}$, C.~F.~Redmer$^{35}$, K.~J.~Ren$^{39}$, A.~Rivetti$^{73c}$, V.~Rodin$^{63}$, M.~Rolo$^{73c}$, G.~Rong$^{1,62}$, Ch.~Rosner$^{18}$, S.~N.~Ruan$^{43}$, N.~Salone$^{44}$, A.~Sarantsev$^{36,c}$, Y.~Schelhaas$^{35}$, K.~Schoenning$^{74}$, M.~Scodeggio$^{29a,29b}$, K.~Y.~Shan$^{13,f}$, W.~Shan$^{24}$, X.~Y.~Shan$^{70,57}$, J.~F.~Shangguan$^{54}$, L.~G.~Shao$^{1,62}$, M.~Shao$^{70,57}$, C.~P.~Shen$^{13,f}$, H.~F.~Shen$^{1,62}$, W.~H.~Shen$^{62}$, X.~Y.~Shen$^{1,62}$, B.~A.~Shi$^{62}$, H.~C.~Shi$^{70,57}$, J.~L.~Shi$^{13}$, J.~Y.~Shi$^{1}$, Q.~Q.~Shi$^{54}$, R.~S.~Shi$^{1,62}$, X.~Shi$^{1,57}$, J.~J.~Song$^{19}$, T.~Z.~Song$^{58}$, W.~M.~Song$^{34,1}$, Y. ~J.~Song$^{13}$, Y.~X.~Song$^{46,g}$, S.~Sosio$^{73a,73c}$, S.~Spataro$^{73a,73c}$, F.~Stieler$^{35}$, Y.~J.~Su$^{62}$, G.~B.~Sun$^{75}$, G.~X.~Sun$^{1}$, H.~Sun$^{62}$, H.~K.~Sun$^{1}$, J.~F.~Sun$^{19}$, K.~Sun$^{60}$, L.~Sun$^{75}$, S.~S.~Sun$^{1,62}$, T.~Sun$^{1,62}$, W.~Y.~Sun$^{34}$, Y.~Sun$^{10}$, Y.~J.~Sun$^{70,57}$, Y.~Z.~Sun$^{1}$, Z.~T.~Sun$^{49}$, Y.~X.~Tan$^{70,57}$, C.~J.~Tang$^{53}$, G.~Y.~Tang$^{1}$, J.~Tang$^{58}$, Y.~A.~Tang$^{75}$, L.~Y~Tao$^{71}$, Q.~T.~Tao$^{25,h}$, M.~Tat$^{68}$, J.~X.~Teng$^{70,57}$, V.~Thoren$^{74}$, W.~H.~Tian$^{58}$, W.~H.~Tian$^{51}$, Y.~Tian$^{31,62}$, Z.~F.~Tian$^{75}$, I.~Uman$^{61b}$, S.~J.~Wang $^{49}$, B.~Wang$^{1}$, B.~L.~Wang$^{62}$, Bo~Wang$^{70,57}$, C.~W.~Wang$^{42}$, D.~Y.~Wang$^{46,g}$, F.~Wang$^{71}$, H.~J.~Wang$^{38,j,k}$, H.~P.~Wang$^{1,62}$, J.~P.~Wang $^{49}$, K.~Wang$^{1,57}$, L.~L.~Wang$^{1}$, M.~Wang$^{49}$, Meng~Wang$^{1,62}$, S.~Wang$^{13,f}$, S.~Wang$^{38,j,k}$, T. ~Wang$^{13,f}$, T.~J.~Wang$^{43}$, W.~Wang$^{58}$, W. ~Wang$^{71}$, W.~P.~Wang$^{70,57}$, X.~Wang$^{46,g}$, X.~F.~Wang$^{38,j,k}$, X.~J.~Wang$^{39}$, X.~L.~Wang$^{13,f}$, Y.~Wang$^{60}$, Y.~D.~Wang$^{45}$, Y.~F.~Wang$^{1,57,62}$, Y.~H.~Wang$^{47}$, Y.~N.~Wang$^{45}$, Y.~Q.~Wang$^{1}$, Yaqian~Wang$^{17,1}$, Yi~Wang$^{60}$, Z.~Wang$^{1,57}$, Z.~L. ~Wang$^{71}$, Z.~Y.~Wang$^{1,62}$, Ziyi~Wang$^{62}$, D.~Wei$^{69}$, D.~H.~Wei$^{15}$, F.~Weidner$^{67}$, S.~P.~Wen$^{1}$, C.~W.~Wenzel$^{4}$, U.~Wiedner$^{4}$, G.~Wilkinson$^{68}$, M.~Wolke$^{74}$, L.~Wollenberg$^{4}$, C.~Wu$^{39}$, J.~F.~Wu$^{1,62}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{1,62}$, X.~Wu$^{13,f}$, X.~H.~Wu$^{34}$, Y.~Wu$^{70}$, Y.~J.~Wu$^{31}$, Z.~Wu$^{1,57}$, L.~Xia$^{70,57}$, X.~M.~Xian$^{39}$, T.~Xiang$^{46,g}$, D.~Xiao$^{38,j,k}$, G.~Y.~Xiao$^{42}$, S.~Y.~Xiao$^{1}$, Y. ~L.~Xiao$^{13,f}$, Z.~J.~Xiao$^{41}$, C.~Xie$^{42}$, X.~H.~Xie$^{46,g}$, Y.~Xie$^{49}$, Y.~G.~Xie$^{1,57}$, Y.~H.~Xie$^{7}$, Z.~P.~Xie$^{70,57}$, T.~Y.~Xing$^{1,62}$, C.~F.~Xu$^{1,62}$, C.~J.~Xu$^{58}$, G.~F.~Xu$^{1}$, H.~Y.~Xu$^{65}$, Q.~J.~Xu$^{16}$, Q.~N.~Xu$^{30}$, W.~Xu$^{1,62}$, W.~L.~Xu$^{65}$, X.~P.~Xu$^{54}$, Y.~C.~Xu$^{77}$, Z.~P.~Xu$^{42}$, Z.~S.~Xu$^{62}$, F.~Yan$^{13,f}$, L.~Yan$^{13,f}$, W.~B.~Yan$^{70,57}$, W.~C.~Yan$^{80}$, X.~Q.~Yan$^{1}$, H.~J.~Yang$^{50,e}$, H.~L.~Yang$^{34}$, H.~X.~Yang$^{1}$, Tao~Yang$^{1}$, Y.~Yang$^{13,f}$, Y.~F.~Yang$^{43}$, Y.~X.~Yang$^{1,62}$, Yifan~Yang$^{1,62}$, Z.~W.~Yang$^{38,j,k}$, Z.~P.~Yao$^{49}$, M.~Ye$^{1,57}$, M.~H.~Ye$^{9}$, J.~H.~Yin$^{1}$, Z.~Y.~You$^{58}$, B.~X.~Yu$^{1,57,62}$, C.~X.~Yu$^{43}$, G.~Yu$^{1,62}$, J.~S.~Yu$^{25,h}$, T.~Yu$^{71}$, X.~D.~Yu$^{46,g}$, C.~Z.~Yuan$^{1,62}$, L.~Yuan$^{2}$, S.~C.~Yuan$^{1}$, X.~Q.~Yuan$^{1}$, Y.~Yuan$^{1,62}$, Z.~Y.~Yuan$^{58}$, C.~X.~Yue$^{39}$, A.~A.~Zafar$^{72}$, F.~R.~Zeng$^{49}$, X.~Zeng$^{13,f}$, Y.~Zeng$^{25,h}$, Y.~J.~Zeng$^{1,62}$, X.~Y.~Zhai$^{34}$, Y.~C.~Zhai$^{49}$, Y.~H.~Zhan$^{58}$, A.~Q.~Zhang$^{1,62}$, B.~L.~Zhang$^{1,62}$, B.~X.~Zhang$^{1}$, D.~H.~Zhang$^{43}$, G.~Y.~Zhang$^{19}$, H.~Zhang$^{70}$, H.~H.~Zhang$^{58}$, H.~H.~Zhang$^{34}$, H.~Q.~Zhang$^{1,57,62}$, H.~Y.~Zhang$^{1,57}$, J.~Zhang$^{80}$, J.~J.~Zhang$^{51}$, J.~L.~Zhang$^{20}$, J.~Q.~Zhang$^{41}$, J.~W.~Zhang$^{1,57,62}$, J.~X.~Zhang$^{38,j,k}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,62}$, Jianyu~Zhang$^{62}$, Jiawei~Zhang$^{1,62}$, L.~M.~Zhang$^{60}$, L.~Q.~Zhang$^{58}$, Lei~Zhang$^{42}$, P.~Zhang$^{1,62}$, Q.~Y.~~Zhang$^{39,80}$, Shuihan~Zhang$^{1,62}$, Shulei~Zhang$^{25,h}$, X.~D.~Zhang$^{45}$, X.~M.~Zhang$^{1}$, X.~Y.~Zhang$^{49}$, Xuyan~Zhang$^{54}$, Y. ~Zhang$^{71}$, Y.~Zhang$^{68}$, Y. ~T.~Zhang$^{80}$, Y.~H.~Zhang$^{1,57}$, Yan~Zhang$^{70,57}$, Yao~Zhang$^{1}$, Z.~H.~Zhang$^{1}$, Z.~L.~Zhang$^{34}$, Z.~Y.~Zhang$^{75}$, Z.~Y.~Zhang$^{43}$, G.~Zhao$^{1}$, J.~Zhao$^{39}$, J.~Y.~Zhao$^{1,62}$, J.~Z.~Zhao$^{1,57}$, Lei~Zhao$^{70,57}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{43}$, S.~J.~Zhao$^{80}$, Y.~B.~Zhao$^{1,57}$, Y.~X.~Zhao$^{31,62}$, Z.~G.~Zhao$^{70,57}$, A.~Zhemchugov$^{36,a}$, B.~Zheng$^{71}$, J.~P.~Zheng$^{1,57}$, W.~J.~Zheng$^{1,62}$, Y.~H.~Zheng$^{62}$, B.~Zhong$^{41}$, X.~Zhong$^{58}$, H. ~Zhou$^{49}$, L.~P.~Zhou$^{1,62}$, X.~Zhou$^{75}$, X.~K.~Zhou$^{7}$, X.~R.~Zhou$^{70,57}$, X.~Y.~Zhou$^{39}$, Y.~Z.~Zhou$^{13,f}$, J.~Zhu$^{43}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,57,62}$, L.~Zhu$^{34}$, L.~X.~Zhu$^{62}$, S.~H.~Zhu$^{69}$, S.~Q.~Zhu$^{42}$, T.~J.~Zhu$^{13,f}$, W.~J.~Zhu$^{13,f}$, Y.~C.~Zhu$^{70,57}$, Z.~A.~Zhu$^{1,62}$, J.~H.~Zou$^{1}$, J.~Zu$^{70,57}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Beijing Institute of Petrochemical Technology, Beijing 102617, People's Republic of China\\
$^{4}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{5}$ Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{6}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{7}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{8}$ Central South University, Changsha 410083, People's Republic of China\\
$^{9}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{10}$ China University of Geosciences, Wuhan 430074, People's Republic of China\\
$^{11}$ Chung-Ang University, Seoul, 06974, Republic of Korea\\
$^{12}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{13}$ Fudan University, Shanghai 200433, People's Republic of China\\
$^{14}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{15}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{16}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{17}$ Hebei University, Baoding 071002, People's Republic of China\\
$^{18}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{19}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{20}$ Henan University, Kaifeng 475004, People's Republic of China\\
$^{21}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{22}$ Henan University of Technology, Zhengzhou 450001, People's Republic of China\\
$^{23}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{24}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{25}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{26}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{27}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{28a}$ INFN Laboratori Nazionali di Frascati, INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy\\
$^{28b}$ INFN Sezione di Perugia, I-06100, Perugia, Italy\\
$^{28c}$ University of Perugia, I-06100, Perugia, Italy\\
$^{29a}$ INFN Sezione di Ferrara, INFN Sezione di Ferrara, I-44122, Ferrara, Italy\\
$^{29b}$ University of Ferrara, I-44122, Ferrara, Italy\\
$^{30}$ Inner Mongolia University, Hohhot 010021, People's Republic of China\\
$^{31}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{32}$ Institute of Physics and Technology, Peace Avenue 54B, Ulaanbaatar 13330, Mongolia\\
$^{33}$ Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Casilla 7D, Arica 1000000, Chile\\
$^{34}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{35}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{36}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{37}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{38}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{39}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{40}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{41}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{42}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{43}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{44}$ National Centre for Nuclear Research, Warsaw 02-093, Poland\\
$^{45}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{46}$ Peking University, Beijing 100871, People's Republic of China\\
$^{47}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{48}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{49}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{50}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{51}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{52}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{53}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{54}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{55}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{56}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{57}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{58}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{59}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{60}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{61a}$ Turkish Accelerator Center Particle Factory Group, Istinye University, 34010, Istanbul, Turkey\\
$^{61b}$ Near East University, Nicosia, North Cyprus, 99138, Mersin 10, Turkey\\
$^{62}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{63}$ University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{64}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{65}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{66}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{67}$ University of Muenster, Wilhelm-Klemm-Strasse 9, 48149 Muenster, Germany\\
$^{68}$ University of Oxford, Keble Road, Oxford OX13RH, United Kingdom\\
$^{69}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{70}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{71}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{72}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{73a}$ University of Turin and INFN, University of Turin, I-10125, Turin, Italy\\
$^{73b}$ University of Eastern Piedmont, I-15121, Alessandria, Italy\\
$^{73c}$ INFN, I-10125, Turin, Italy\\
$^{74}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{75}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{76}$ Xinyang Normal University, Xinyang 464000, People's Republic of China\\
$^{77}$ Yantai University, Yantai 264005, People's Republic of China\\
$^{78}$ Yunnan University, Kunming 650500, People's Republic of China\\
$^{79}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{80}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{b}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{c}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{d}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{e}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{f}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{g}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{h}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{i}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{j}$ Also at MOE Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{k}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{l}$ Also at the Department of Mathematical Sciences, IBA, Karachi 75270, Pakistan\\
}\end{center}
\vspace{0.4cm}
\end{small}
}

